Insights into the Production of $^{44}$Ti and Nickel Isotopes in Core-Collapse Supernovae

We report nucleosynthetic results for both $^{44}$Ti and nickel isotopes for eighteen three-dimensional (3D) core-collapse supernova (CCSN) simulations extended to $\sim$20 seconds after bounce. We find that many of our long-term models are able to achieve $^{44}$Ti/$^{56}$Ni ratios similar to that observed in Cassiopeia A, and modern supernova models can synthesize up to $2\times10^{-4}M_\odot$ of $^{44}$Ti. Neutrino-driven winds and the fact that there can be simultaneous accretion and explosion in 3D models of core-collapse supernovae play central roles in its production. We conclude that the $^{44}$Ti underproduction problem in previous CCSN models is no longer an issue. In addition, we discuss the production of both $^{57}$Ni and stable nickel/iron ratios and compare our results to observations of SN1987A and the Crab.

==> trash.tex <==
\section{Ejecta Components}\label{sec:components}
freeze-out vs explosive nucleosynthesis. Dependence upon various explosion properties. What's the mass ratio between freeze-out and explosive components? Is it a constant? 

3D rendering figure: low mass early spherical explosion vs high mass late asymmetrical explosion. Also show the transition between wind region (or freeze-out region) and explosive region.

Figure of electron fraction evolution: early explosion, ye start from neutron rich. late explosion, ye start from proton rich. 

Figure of ejecta abundance and production factor. early vs late explosions.
